Focusing on Context is NICE: Improving Overshadowed Entity Disambiguation

Entity disambiguation (ED) is the task of mapping an ambiguous entity mention to the corresponding entry in a structured knowledge base. Previous research showed that entity overshadowing is a significant challenge for existing ED models: when presented with an ambiguous entity mention, the models are much more likely to rank a more frequent yet less contextually relevant entity at the top. Here, we present NICE, an iterative approach that uses entity type information to leverage context and avoid over-relying on the frequency-based prior. Our experiments show that NICE achieves the best performance results on the overshadowed entities while still performing competitively on the frequent entities.

==> _outline.tex <==
(This is an outline in questions. We'll turn it into proper text once the storyline is clear.) \\\\
%
Q: What do we want? \\
A: We want to improve entity linking on overshadowed entities. \\\\
%
Q: Wait, what is entity linking and what are overshadowed entities? \\
A: Fine, I'll insert the definitions here. \\\\
%
Q: That's better. So, how do we want to improve EL for overshadowed entities? \\
A: EL is still a challenging task, ShadowLink \cite{shadowlink} proves it.  And overshadowed entities are frequent (show some numbers: N ambiguous entities in Wikidata, for each "top" entity there is at least one overshadowed entity) \\\\
%
Q: Ok, how do we make it work? \\
A: We want to pay more attention to the context on the KG level and improve the coherence. A document usually contains multiple entities, so when disambiguating a target entity, we'll look which candidate is closer to other entities that we have already disambiguated. We'll insert a picture with an example here (Odessa or something similar). \\\\
%
Q: Seems clear. What's next? \\
A: Let's talk about our methods.\\\\

Q: So, what do we use to improve entity linking on overshadowed entities by paying more attention to the context? \\
A: We move iteratively. First, we find an entity that has the least number of candidates. \\\\
%
Q: Technically, every entity could have many candidates (depends on the search method) – how do you know when you've seen all relevant candidates for the least ambiguous entity? \\
A: We'll pick some threshold and use string matching. \\\\
%
Q: How exactly? \\
A: If a candidate contains our mention as a substring (with some degree of possible fuzziness), it's a good one. If not, screw it! \\\\
%
Q: How do we implement fuzzy substring matching? \\
A: Let's use fuzz.partial\_ratio from the FuzzyWuzzy library. If the ratio is above 80 (for example), the candidate is OK. \\ \\
%
Q: Sounds like it might work. But how do we retrieve the candidates in the first place? \\
A: We can use either REL or GENRE. REL is fast, GENRE is much slower but more precise - we can play around and see what's more realistic. \\\\
%
Q: Fine, we've retreived all the candidates, sorted the entities by their ambiguity and picked the least ambiguous one. What's next? \\
A: We disambiguate the first entity using priors, and then go iteratively: for each new entity, choose a candidate which is the closest to already disambiguated entities.\\\\
%
Q: The method looks simple and pretty elegant. Has anybody done this before? \\
A: I have no idea! Let's look at SOTA: if none of the famous algorithms does exactly that, we can assume that it hasn't been done before. If we find something similar, we can see how to improve it.  My assumption is that it definitely exists somewhere, but it was probably invented long ago, and the EL methods - both candidate retrieval and measuring similarity - have improved a lot since then. \\\\
%
Q: Oh, about that: how do we measure the distance between entities? \\
A: We will try different things. WAT relatedness API offers different metrics. The ones that lead to the best improvements in the preliminary experiments are Milne-Witten, Barabasi-Albert, and Word2Vec – but we'll double-check it. There are also at least two different ways to aggregate the distance: average and maximum. \\\\
%
Q: Are we only going to use WAT's metrics for entity relatedness? \\
A: An interesting idea would be to also play around with message passing, but it will take a bit of time for me to understand.

METHODS

Add a picture: TagMe for mention detection, REL for candidate generation, NICE for collective disambiguation
ICE algorithm description here
\begin{algorithm}
\caption{An algorithm example with caption}\label{alg:cap}
\begin{algorithmic}
\Require $n \geq 0$
\Ensure $y = x^n$
\State $y \gets 1$
\State $X \gets x$
\State $N \gets n$
\While{$N \neq 0$}
\If{$N$ is even}
    \State $X \gets X \times X$
    \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
\ElsIf{$N$ is odd}
    \State $y \gets y \times X$
    \State $N \gets N - 1$
\EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}

goal: Improve ED for overshadowed entities
\\%
how: Get better at using relatedness (as opposed to commonness, aka prior)
what's in relatedness: Mention-entity similarity + context-entity similarity + entity-entity similarity (aka entity coherence)
\\%
ways to capture mention-entity similarity: Word embeddings (of a mention and its candidate entity); NER-based filtering of candidates; other ways to filter candidates ...
\\%
ways to capture context-entity similarity: Word embeddings (of the context, i.e. part of the sentence, and a candidate entity – that's what REL does); possibly other things
\\%
ways to capture entity-entity similarity: Word embeddings; graph embeddings; graph-based metrics: Milne-Witten, PMI, Barabasi-Albert, Jaccard measure of pages outlinks; message-passing on KG; possibly other things

Q: Which dataset do we use to evaluate our models? \\
A: An obvious choice is ShadowLink: the first dataset designed specifically for overshadowed entities. Then we can add AmbER which was constructed in a similar way. To evaluate on AmbER, we need some extra work (converting it to GERBIL-friendly NIF format), but it should be fine. \\\\
%
Q: Which metrics do we use?\\
A: The classics: P, R, F. \\\\
%
Q: Which baselines do we compare to?\\
A: Everything from the ShadowLink paper plus 3 extra baselines: ner4el, eigenthemes and Bootleg. The latter was designed for tail entities, which is not exactly the same as overshadowed but close, so makes sense to include it.

==> scrap.tex <==

\begin{algorithm}
    \caption{ICE disambiguation}
    \label{alg:ice}
\small
\setstretch{1.35}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwInOut{Where}{~}
	\DontPrintSemicolon
    \Input{$S_{todo} = \{{ment}_i: cands_i\}_{i=1}^n$ \\ where~$cands_i = [{cand}^1_i, ..., {cand}^{k_i}_i]$}
    \Output{$S_{ans} = \{{ment}_i:  {cand}^*_i\}_{i=1}^n$}
    \tcp{Part 1. Seed entity disambiguation}
        $m_{seed} \leftarrow find\_least\_ambiguous(S_{todo})$\\
        $S_{todo} \leftarrow S_{todo} \setminus \{m_{seed}, cands_{seed}\}$ \\
        $cand_{seed} \leftarrow disamb\_seed(m_{seed}, cands_{seed})$ \\
        $S_{ans} \leftarrow S_{ans} \cup \{m_{seed}, cand^*_{seed}\}$ \\
        \tcc{Seed entity disambiguation ends}
    % }
    % \Collective{
    \tcp{Part 2. Collective disambiguation}
        \While{$S_{todo} \neq \emptyset$} {
          $m_i \leftarrow find\_least\_ambiguous(S_{todo})$ \\
         $S_{todo} \leftarrow S_{todo} \setminus \{m_i, cands_i\}$ \\
         \tcp{Choose the candidate closest to the already disambiguated entities} \\
         $cand^*_i \leftarrow argmax~aggr\_rel(cands_i, S_{ans})$ \\
         $S_{ans} \leftarrow S_{ans} \cup \{m_i, cand^*_i\}$\\
    % }\\
    % \tcc{One candidate per mention}
\end{algorithm}

AIDA-like: $a_1*score_{ICE}+a_2*score_{NER4EL}+a_3*prior$

\begin{table}[!h]
\resizebox{\columnwidth}{!}{%
    \centering
    \begin{tabular}{@{}lrrr@{}}
    \toprule
    Baseline & pred(top) != pred(shadow), \% & pred(top) is correct, \% & pred(shadow) is correct, \% \\ \midrule
    AIDA & \textbf{26.7} & 67.8 & 43.5 \\
    WAT & 29.2 & 59.2 & 28.4 \\
    REL & 56.5 & {\ul 70.0} & 27.2 \\
    GENRE & 35.5 & 53.7 & 34.2 \\
    NER4EL & 43.0 & 68.9 & {\ul 45.7} \\ \midrule
    NICE & 28.4 &  &  \\ \bottomrule
    \end{tabular}
    \caption{\label{tbl:overshadowing} Overshadowing}
}
\end{table}

The predicted NER types are shown under the corresponding entity mentions. The candidates with a NER type different from the predicted ones are discarded, while others (in bold) are kept.



\begin{figure}[h!]
    % \centering
    \includegraphics[width=\columnwidth, height=6cm,keepaspectratio]{figures/overshadowing_by_baseline.png}
    \caption{Entity overshadowing and context sensitivity of the methods under evaluation} 
    \label{fig:baselines_overshadowing}
\end{figure}
\subsection{The impact of overshadowing} To measure the impact of entity overshadowing and estimate context sensitivity of the models, we perform a robustness evaluation. By definition, overshadowing impacts ED performance when a model outputs the same answer for two different entities that share the same surface form, and one of the two entities is more frequent than the other. The number of predictions affected by overshadowing can be seen as a proxy for measuring context sensitivity of a model: if a model tends to present the same answer for the same entity surface form in different context, it is likely to be suffering from over-relying on prior predictions.

We measure how often this occurs on the filtered Top and Shadow subsets of the ShadowLink dataset, both for the NICE method and for all of the baselines under evaluation. To do so, we downsampled the filtered subsets, keeping the entries for which the entity surface form is seen both in Top-filtered and Shadow-filtered, which resulted in 363 Top and 363 Shadow entries linked together by shared surface forms. We then compare the predictions of all methods on these two subsets, counting the number of times when a prediction for a Top entity coincided with the prediction for the corresponding Shadow entity.
The results are presented in Figure~\ref{fig:baselines_overshadowing}: for every system it is shown how many answers were \textbf{not} affected by overshadowing, how many answers were correct on the Top sample and how many answers were correct on the Shadow sample.  From the results it can seen that the models  ... (more about this: NICE is as "context-sensitive" as WAT and AIDA; low context sensitivity means poor results on Shadow, but not all wrong answers are caused by overshadowing
)
